Role of magnetic fields in fueling Seyfert nuclei

Molecular gas is believed to be the fuel for star formation and nuclear activity in Seyfert galaxies. To explore the role of magnetic fields in funneling molecular gas into the nuclear region, measurements of the magnetic fields embedded in molecular gas are needed. By applying the new velocity gradient technique (VGT) to ALMA and PAWS's CO isotopolog data, we obtain the first detection of CO-associated magnetic fields in several nearby Seyfert galaxies and their unprecedented high-resolution magnetic field maps. The VGT-measured magnetic fields in molecular gas globally agree with those inferred from existing HAWC+ dust polarization and VLA synchrotron polarization. An overall good alignment between the magnetic fields traced by VGT-CO and by synchrotron polarization may support the correlation between star formation and cosmic ray generation. We find that the magnetic fields traced by VGT-CO have a significant radial component in the central regions of most Seyferts in our sample, where efficient molecular gas inflows or outflows may happen. In particular, we find local misalignment between the magnetic fields traced by CO and dust polarization within the nuclear ring of NGC 1097, and the former aligns with the central bar's orientation. This misalignment reveals different magnetic field configurations in different gas phases and may provide an observational diagnostic for the ongoing multi-phase fueling of Seyfert activity.

==> sample <==
@ARTICLE{2017ApJ...835...41G,
       author = {{Gonz{\'a}lez-Casanova}, Diego F. and {Lazarian}, A.},
        title = "{Velocity Gradients as a Tracer for Magnetic Fields}",
      journal = {ApJ},
     keywords = {ISM: kinematics and dynamics, ISM: magnetic fields, magnetohydrodynamics: MHD, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = jan,
       volume = {835},
       number = {1},
          eid = {41},
        pages = {41},
          doi = {10.3847/1538-4357/835/1/41},
archivePrefix = {arXiv},
       eprint = {arXiv:1608.06867},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...835...41G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Garc03,
       author = {{Garc{\'\i}a-Burillo}, S. and {Combes}, F. and {Hunt}, L.~K. and {Boone}, F. and {Baker}, A.~J. and {Tacconi}, L.~J. and {Eckart}, A. and {Neri}, R. and {Leon}, S. and {Schinnerer}, E. and {Englmaier}, P.},
        title = "{Molecular Gas in NUclei of GAlaxies (NUGA). I. The counter-rotating LINER NGC 4826}",
      journal = {AA},
     keywords = {galaxies: individual: NGC 4826, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, radio lines: galaxies, Astrophysics},
         year = 2003,
        month = aug,
       volume = {407},
        pages = {485-502},
          doi = {10.1051/0004-6361:20030866},
archivePrefix = {arXiv},
       eprint = {astro-ph/0306140},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...407..485G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Moss01,
       author = {{Moss}, D. and {Shukurov}, A. and {Sokoloff}, D. and {Beck}, R. and {Fletcher}, A.},
        title = "{Magnetic fields in barred galaxies. II. Dynamo models}",
      journal = {AA},
     keywords = {MAGNETIC FIELDS, MHD, GALAXIES: SPIRAL, GALAXIES: ISM, GALAXIES: MAGNETIC FIELDS, GALAXIES: INDIVIDUAL: NGC 1097, Astrophysics},
         year = 2001,
        month = dec,
       volume = {380},
        pages = {55-71},
          doi = {10.1051/0004-6361:20011343},
archivePrefix = {arXiv},
       eprint = {astro-ph/0107214},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...380...55M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Beck96,
       author = {{Beck}, Rainer and {Brandenburg}, Axel and {Moss}, David and {Shukurov}, Anvar and {Sokoloff}, Dmitry},
        title = "{Galactic Magnetism: Recent Developments and Perspectives}",
      journal = {ARAA},
         year = 1996,
        month = jan,
       volume = {34},
        pages = {155-206},
          doi = {10.1146/annurev.astro.34.1.155},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ARA&A..34..155B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Wada04,
       author = {{Wada}, Keiichi},
        title = "{Fueling Gas to the Central Region of Galaxies}",
     keywords = {Astrophysics},
    booktitle = {Coevolution of Black Holes and Galaxies},
         year = 2004,
       editor = {{Ho}, Luis C.},
        month = jan,
        pages = {186},
archivePrefix = {arXiv},
       eprint = {astro-ph/0308134},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004cbhg.symp..186W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Ching22,
       author = {{Ching}, T. -C. and {Li}, D. and {Heiles}, C. and {Li}, Z. -Y. and {Qian}, L. and {Yue}, Y.~L. and {Tang}, J. and {Jiao}, S.~H.},
        title = "{An early transition to magnetic supercriticality in star formation}",
      journal = {Nature},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = jan,
       volume = {601},
       number = {7891},
        pages = {49-52},
          doi = {10.1038/s41586-021-04159-x},
archivePrefix = {arXiv},
       eprint = {arXiv:2112.12644},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022Natur.601...49C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{XL22,
       author = {{Xu}, Siyao and {Lazarian}, Alex},
        title = "{Cosmic Ray Streaming in the Turbulent Interstellar Medium}",
      journal = {ApJ},
     keywords = {Galactic cosmic rays, Magnetohydrodynamics, Interstellar medium, 567, 1964, 847, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Astrophysics of Galaxies, Physics - Plasma Physics},
         year = 2022,
        month = mar,
       volume = {927},
       number = {1},
          eid = {94},
        pages = {94},
          doi = {10.3847/1538-4357/ac4dfd},
archivePrefix = {arXiv},
       eprint = {arXiv:2112.06941},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJ...927...94X},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Planck14,
       author = {{Planck Collaboration} and {Ade}, P.~A.~R. and {Aghanim}, N. and {Alves}, M.~I.~R. and {Armitage-Caplan}, C. and {Arnaud}, M. and {Ashdown}, M. and {Atrio-Barandela}, F. and {Aumont}, J. and {Aussel}, H. and {Baccigalupi}, C. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Barrena}, R. and {Bartelmann}, M. and {Bartlett}, J.~G. and {Bartolo}, N. and {Basak}, S. and {Battaner}, E. and {Battye}, R. and {Benabed}, K. and {Beno{\^\i}t}, A. and {Benoit-L{\'e}vy}, A. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bertincourt}, B. and {Bethermin}, M. and {Bielewicz}, P. and {Bikmaev}, I. and {Blanchard}, A. and {Bobin}, J. and {Bock}, J.~J. and {B{\"o}hringer}, H. and {Bonaldi}, A. and {Bonavera}, L. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bourdin}, H. and {Bowyer}, J.~W. and {Bridges}, M. and {Brown}, M.~L. and {Bucher}, M. and {Burenin}, R. and {Burigana}, C. and {Butler}, R.~C. and {Calabrese}, E. and {Cappellini}, B. and {Cardoso}, J. -F. and {Carr}, R. and {Carvalho}, P. and {Casale}, M. and {Castex}, G. and {Catalano}, A. and {Challinor}, A. and {Chamballu}, A. and {Chary}, R. -R. and {Chen}, X. and {Chiang}, H.~C. and {Chiang}, L. -Y. and {Chon}, G. and {Christensen}, P.~R. and {Churazov}, E. and {Church}, S. and {Clemens}, M. and {Clements}, D.~L. and {Colombi}, S. and {Colombo}, L.~P.~L. and {Combet}, C. and {Comis}, B. and {Couchot}, F. and {Coulais}, A. and {Crill}, B.~P. and {Cruz}, M. and {Curto}, A. and {Cuttaia}, F. and {Da Silva}, A. and {Dahle}, H. and {Danese}, L. and {Davies}, R.~D. and {Davis}, R.~J. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {D{\'e}chelette}, T. and {Delabrouille}, J. and {Delouis}, J. -M. and {D{\'e}mocl{\`e}s}, J. and {D{\'e}sert}, F. -X. and {Dick}, J. and {Dickinson}, C. and {Diego}, J.~M. and {Dolag}, K. and {Dole}, H. and {Donzelli}, S. and {Dor{\'e}}, O. and {Douspis}, M. and {Ducout}, A. and {Dunkley}, J. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Fabre}, O. and {Falgarone}, E. and {Falvella}, M.~C. and {Fantaye}, Y. and {Fergusson}, J. and {Filliard}, C. and {Finelli}, F. and {Flores-Cacho}, I. and {Foley}, S. and {Forni}, O. and {Fosalba}, P. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Freschi}, M. and {Fromenteau}, S. and {Frommert}, M. and {Gaier}, T.~C. and {Galeotta}, S. and {Gallegos}, J. and {Galli}, S. and {Gandolfo}, B. and {Ganga}, K. and {Gauthier}, C. and {G{\'e}nova-Santos}, R.~T. and {Ghosh}, T. and {Giard}, M. and {Giardino}, G. and {Gilfanov}, M. and {Girard}, D. and {Giraud-H{\'e}raud}, Y. and {Gjerl{\o}w}, E. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gregorio}, A. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Haissinski}, J. and {Hamann}, J. and {Hansen}, F.~K. and {Hansen}, M. and {Hanson}, D. and {Harrison}, D.~L. and {Heavens}, A. and {Helou}, G. and {Hempel}, A. and {Henrot-Versill{\'e}}, S. and {Hern{\'a}ndez-Monteagudo}, C. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Hivon}, E. and {Ho}, S. and {Hobson}, M. and {Holmes}, W.~A. and {Hornstrup}, A. and {Hou}, Z. and {Hovest}, W. and {Huey}, G. and {Huffenberger}, K.~M. and {Hurier}, G. and {Ili{\'c}}, S. and {Jaffe}, A.~H. and {Jaffe}, T.~R. and {Jasche}, J. and {Jewell}, J. and {Jones}, W.~C. and {Juvela}, M. and {Kalberla}, P. and {Kangaslahti}, P. and {Keih{\"a}nen}, E. and {Kerp}, J. and {Keskitalo}, R. and {Khamitov}, I. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Kneissl}, R. and {Knoche}, J. and {Knox}, L. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lacasa}, F. and {Lagache}, G. and {L{\"a}hteenm{\"a}ki}, A. and {Lamarre}, J. -M. and {Langer}, M. and {Lasenby}, A. and {Lattanzi}, M. and {Laureijs}, R.~J. and {Lavabre}, A. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Leach}, S. and {Leahy}, J.~P. and {Leonardi}, R. and {Le{\'o}n-Tavares}, J. and {Leroy}, C. and {Lesgourgues}, J. and {Lewis}, A. and {Li}, C. and {Liddle}, A. and {Liguori}, M. and {Lilje}, P.~B. and {Linden-V{\o}rnle}, M. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lowe}, S. and {Lubin}, P.~M. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {MacTavish}, C.~J. and {Maffei}, B. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Marinucci}, D. and {Maris}, M. and {Marleau}, F. and {Marshall}, D.~J. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Masi}, S. and {Massardi}, M. and {Matarrese}, S. and {Matsumura}, T. and {Matthai}, F. and {Maurin}, L. and {Mazzotta}, P. and {McDonald}, A. and {McEwen}, J.~D. and {McGehee}, P. and {Mei}, S. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Melin}, J. -B. and {Mendes}, L. and {Menegoni}, E. and {Mennella}, A. and {Migliaccio}, M. and {Mikkelsen}, K. and {Millea}, M. and {Miniscalco}, R. and {Mitra}, S. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Morisset}, N. and {Mortlock}, D. and {Moss}, A. and {Munshi}, D. and {Murphy}, J.~A. and {Naselsky}, P. and {Nati}, F. and {Natoli}, P. and {Negrello}, M. and {Nesvadba}, N.~P.~H. and {Netterfield}, C.~B. and {N{\o}rgaard-Nielsen}, H.~U. and {North}, C. and {Noviello}, F. and {Novikov}, D. and {Novikov}, I. and {O'Dwyer}, I.~J. and {Orieux}, F. and {Osborne}, S. and {O'Sullivan}, C. and {Oxborrow}, C.~A. and {Paci}, F. and {Pagano}, L. and {Pajot}, F. and {Paladini}, R. and {Pandolfi}, S. and {Paoletti}, D. and {Partridge}, B. and {Pasian}, F. and {Patanchon}, G. and {Paykari}, P. and {Pearson}, D. and {Pearson}, T.~J. and {Peel}, M. and {Peiris}, H.~V. and {Perdereau}, O. and {Perotto}, L. and {Perrotta}, F. and {Pettorino}, V. and {Piacentini}, F. and {Piat}, M. and {Pierpaoli}, E. and {Pietrobon}, D. and {Plaszczynski}, S. and {Platania}, P. and {Pogosyan}, D. and {Pointecouteau}, E. and {Polenta}, G. and {Ponthieu}, N. and {Popa}, L. and {Poutanen}, T. and {Pratt}, G.~W. and {Pr{\'e}zeau}, G. and {Prunet}, S. and {Puget}, J. -L. and {Pullen}, A.~R. and {Rachen}, J.~P. and {Racine}, B. and {Rahlin}, A. and {R{\"a}th}, C. and {Reach}, W.~T. and {Rebolo}, R. and {Reinecke}, M. and {Remazeilles}, M. and {Renault}, C. and {Renzi}, A. and {Riazuelo}, A. and {Ricciardi}, S. and {Riller}, T. and {Ringeval}, C. and {Ristorcelli}, I. and {Robbers}, G. and {Rocha}, G. and {Roman}, M. and {Rosset}, C. and {Rossetti}, M. and {Roudier}, G. and {Rowan-Robinson}, M. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Rusholme}, B. and {Salerno}, E. and {Sandri}, M. and {Sanselme}, L. and {Santos}, D. and {Savelainen}, M. and {Savini}, G. and {Schaefer}, B.~M. and {Schiavon}, F. and {Scott}, D. and {Seiffert}, M.~D. and {Serra}, P. and {Shellard}, E.~P.~S. and {Smith}, K. and {Smoot}, G.~F. and {Souradeep}, T. and {Spencer}, L.~D. and {Starck}, J. -L. and {Stolyarov}, V. and {Stompor}, R. and {Sudiwala}, R. and {Sunyaev}, R. and {Sureau}, F. and {Sutter}, P. and {Sutton}, D. and {Suur-Uski}, A. -S. and {Sygnet}, J. -F. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Taylor}, D. and {Terenzi}, L. and {Texier}, D. and {Toffolatti}, L. and {Tomasi}, M. and {Torre}, J. -P. and {Tristram}, M. and {Tucci}, M. and {Tuovinen}, J. and {T{\"u}rler}, M. and {Tuttlebee}, M. and {Umana}, G. and {Valenziano}, L. and {Valiviita}, J. and {Van Tent}, B. and {Varis}, J. and {Vibert}, L. and {Viel}, M. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wade}, L.~A. and {Wandelt}, B.~D. and {Watson}, C. and {Watson}, R. and {Wehus}, I.~K. and {Welikala}, N. and {Weller}, J. and {White}, M. and {White}, S.~D.~M. and {Wilkinson}, A. and {Winkel}, B. and {Xia}, J. -Q. and {Yvon}, D. and {Zacchei}, A. and {Zibin}, J.~P. and {Zonca}, A.},
        title = "{Planck 2013 results. I. Overview of products and scientific results}",
      journal = {AA},
     keywords = {cosmology: observations, cosmic background radiation, space vehicles: instruments, instrumentation: detectors, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2014,
        month = nov,
       volume = {571},
          eid = {A1},
        pages = {A1},
          doi = {10.1051/0004-6361/201321529},
archivePrefix = {arXiv},
       eprint = {arXiv:1303.5062},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...571A...1P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Matt21,
       author = {{Matthews}, A.~M. and {Condon}, J.~J. and {Cotton}, W.~D. and {Mauch}, T.},
        title = "{Cosmic Star Formation History Measured at 1.4 GHz}",
      journal = {ApJ},
     keywords = {Galaxy evolution, Cosmological evolution, Star formation, Galaxy counts, Radio galaxies, 594, 336, 1569, 588, 1343, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jun,
       volume = {914},
       number = {2},
          eid = {126},
        pages = {126},
          doi = {10.3847/1538-4357/abfaf6},
archivePrefix = {arXiv},
       eprint = {arXiv:2104.11756},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...914..126M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Zhang93,
       author = {{Zhang}, Xiaolei and {Wright}, Melvyn and {Alexander}, Paul},
        title = "{High-Resolution CO and H I Observations of the Interacting Galaxy NGC 3627}",
      journal = {ApJ},
     keywords = {GALAXIES: EVOLUTION, GALAXIES: INDIVIDUAL NGC NUMBER: NGC 3627, GALAXIES: INTERACTIONS, GALAXIES: ISM, GALAXIES: STRUCTURE},
         year = 1993,
        month = nov,
       volume = {418},
        pages = {100},
          doi = {10.1086/173374},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1993ApJ...418..100Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Colo14,
       author = {{Colombo}, Dario and {Meidt}, Sharon E. and {Schinnerer}, Eva and {Garc{\'\i}a-Burillo}, Santiago and {Hughes}, Annie and {Pety}, J{\'e}r{\^o}me and {Leroy}, Adam K. and {Dobbs}, Clare L. and {Dumas}, Ga{\"e}lle and {Thompson}, Todd A. and {Schuster}, Karl F. and {Kramer}, Carsten},
        title = "{The PdBI Arcsecond Whirlpool Survey (PAWS): Multi-phase Cold Gas Kinematic of M51}",
      journal = {ApJ},
     keywords = {galaxies: individual: M51 NGC 5194, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: spiral, galaxies: structure, ISM: kinematics and dynamics, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2014,
        month = mar,
       volume = {784},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.1088/0004-637X/784/1/4},
archivePrefix = {arXiv},
       eprint = {arXiv:1401.3759},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...784....4C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garca14,
       author = {{Garc{\'\i}a-Burillo}, S. and {Combes}, F. and {Usero}, A. and {Aalto}, S. and {Krips}, M. and {Viti}, S. and {Alonso-Herrero}, A. and {Hunt}, L.~K. and {Schinnerer}, E. and {Baker}, A.~J. and {Boone}, F. and {Casasola}, V. and {Colina}, L. and {Costagliola}, F. and {Eckart}, A. and {Fuente}, A. and {Henkel}, C. and {Labiano}, A. and {Mart{\'\i}n}, S. and {M{\'a}rquez}, I. and {Muller}, S. and {Planesas}, P. and {Ramos Almeida}, C. and {Spaans}, M. and {Tacconi}, L.~J. and {van der Werf}, P.~P.},
        title = "{Molecular line emission in NGC 1068 imaged with ALMA. I. An AGN-driven outflow in the dense molecular gas}",
      journal = {AA},
     keywords = {galaxies: individual: NGC 1068, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jul,
       volume = {567},
          eid = {A125},
        pages = {A125},
          doi = {10.1051/0004-6361/201423843},
archivePrefix = {arXiv},
       eprint = {arXiv:1405.7706},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...567A.125G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Quer16,
       author = {{Querejeta}, M. and {Meidt}, S.~E. and {Schinnerer}, E. and {Garc{\'\i}a-Burillo}, S. and {Dobbs}, C.~L. and {Colombo}, D. and {Dumas}, G. and {Hughes}, A. and {Kramer}, C. and {Leroy}, A.~K. and {Pety}, J. and {Schuster}, K.~F. and {Thompson}, T.~A.},
        title = "{Gravitational torques imply molecular gas inflow towards the nucleus of M 51}",
      journal = {AA},
     keywords = {galaxies: individual: M 51, galaxies: ISM, galaxies: structure, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = apr,
       volume = {588},
          eid = {A33},
        pages = {A33},
          doi = {10.1051/0004-6361/201527536},
archivePrefix = {arXiv},
       eprint = {arXiv:1510.03440},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...588A..33Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wezg12,
       author = {{We{\.z}gowiec}, M. and {Soida}, M. and {Bomans}, D.~J.},
        title = "{NGC 3627: a galaxy-dwarf collision?}",
      journal = {AA},
     keywords = {galaxies: groups: general, galaxies: groups: individual: Leo Triplet, galaxies: individual: NGC 3627, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = aug,
       volume = {544},
          eid = {A113},
        pages = {A113},
          doi = {10.1051/0004-6361/201118436},
archivePrefix = {arXiv},
       eprint = {arXiv:1207.1195},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...544A.113W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Soi01,
       author = {{Soida}, M. and {Urbanik}, M. and {Beck}, R. and {Wielebinski}, R. and {Balkowski}, C.},
        title = "{Unusual magnetic fields in the interacting spiral NGC 3627}",
      journal = {AA},
     keywords = {GALAXIES: MAGNETIC FIELDS, GALAXIES: INTERACTING, GALAXIES: INDIVIDUAL: NGC 3627, RADIO CONTINUUM: GALAXIES, Astrophysics},
         year = 2001,
        month = oct,
       volume = {378},
        pages = {40-50},
          doi = {10.1051/0004-6361:20011185},
archivePrefix = {arXiv},
       eprint = {astro-ph/0109262},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...378...40S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Hay79,
       author = {{Haynes}, M.~P. and {Giovanelli}, R. and {Roberts}, M.~S.},
        title = "{A detailed examination of the neutral hydrogen distribution in the Leo triplet NGC 3632, 3627, and 3628.}",
      journal = {ApJ},
     keywords = {Hydrogen Atoms, Intergalactic Media, Interstellar Gas, Mass Distribution, Spatial Distribution, Astronomical Maps, Galactic Clusters, Gravitational Effects, Tables (Data), Astrophysics, Groups of Galaxies:Intergalactic Gas, Intergalactic Gas},
         year = 1979,
        month = apr,
       volume = {229},
        pages = {83-90},
          doi = {10.1086/156932},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...229...83H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Quil95,
       author = {{Quillen}, A.~C. and {Frogel}, Jay A. and {Kuchinski}, L.~E. and {Terndrup}, D.~M.},
        title = "{Multiband Images of the Barred Galaxy NGC 1097}",
      journal = {AJ},
     keywords = {GALAXIES: INDIVIDUAL: NGC 1079, GALAXIES: ISM, GALAXIES: STELLAR CONTENT, Astrophysics},
         year = 1995,
        month = jul,
       volume = {110},
        pages = {156},
          doi = {10.1086/117503},
archivePrefix = {arXiv},
       eprint = {astro-ph/9503067},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995AJ....110..156Q},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Pata00,
       author = {{Patsis}, P.~A. and {Athanassoula}, E.},
        title = "{SPH simulations of gas flow in barred galaxies. Effect of hydrodynamical and numerical parameters}",
      journal = {AA},
     keywords = {ISM: KINEMATICS AND DYNAMICS, GALAXIES: KINEMATICS AND DYNAMICS, GALAXIES: SPIRAL, GALAXIES: STRUCTURE},
         year = 2000,
        month = jun,
       volume = {358},
        pages = {45-56},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...358...45P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{EngP97,
       author = {{Englmaier}, Peter and {Gerhard}, Ortwin},
        title = "{Two modes of gas flow in a single barred galaxy}",
      journal = {MNRAS},
     keywords = {HYDRODYNAMICS, SHOCK WAVES, ISM: KINEMATICS AND DYNAMICS, GALAXIES: ISM, GALAXIES: SPIRAL, Astrophysics},
         year = 1997,
        month = may,
       volume = {287},
       number = {1},
        pages = {57-68},
          doi = {10.1093/mnras/287.1.57},
archivePrefix = {arXiv},
       eprint = {astro-ph/9611176},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997MNRAS.287...57E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Atha92,
       author = {{Athanassoula}, E.},
        title = "{The existence and shapes of dust lanes in galactic bars.}",
      journal = {MNRAS},
     keywords = {Barred Galaxies, Cosmic Dust, Galactic Rotation, Gas Flow, Stellar Motions, Astronomical Models, Celestial Mechanics, Astrophysics},
         year = 1992,
        month = nov,
       volume = {259},
        pages = {345-364},
          doi = {10.1093/mnras/259.2.345},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992MNRAS.259..345A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{KJ12,
       author = {{Kim}, Woong-Tae and {Stone}, James M.},
        title = "{Two-dimensional Magnetohydrodynamic Simulations of Barred Galaxies}",
      journal = {ApJ},
     keywords = {galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: spiral, ISM: general, magnetohydrodynamics, shock waves, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2012,
        month = jun,
       volume = {751},
       number = {2},
          eid = {124},
        pages = {124},
          doi = {10.1088/0004-637X/751/2/124},
archivePrefix = {arXiv},
       eprint = {arXiv:1204.0073},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...751..124K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Chep10,
       author = {{Chepurnov}, A. and {Lazarian}, A.},
        title = "{Extending the Big Power Law in the Sky with Turbulence Spectra from Wisconsin H{\ensuremath{\alpha}} Mapper Data}",
      journal = {ApJ},
     keywords = {ISM: lines and bands, methods: data analysis, techniques: spectroscopic, turbulence, Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {1},
        pages = {853-858},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Arm95,
       author = {{Armstrong}, J.~W. and {Rickett}, B.~J. and {Spangler}, S.~R.},
        title = "{Electron Density Power Spectrum in the Local Interstellar Medium}",
      journal = {ApJ},
     keywords = {Electron Density Profiles, Interstellar Matter, Power Spectra, Scintillation, Astronomical Models, Plasma Turbulence, Pulsars, Radio Astronomy, Astrophysics, ISM: STRUCTURE, RADIO CONTINUUM: ISM, STARS: PULSARS: GENERAL, TURBULENCE},
         year = 1995,
        month = apr,
       volume = {443},
        pages = {209},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2020A&A...641A..11P,
       author = {{Planck Collaboration} and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bernard}, J. -P. and {Bersanelli}, M. and {Bielewicz}, P. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bracco}, A. and {Bucher}, M. and {Burigana}, C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Chiang}, H.~C. and {Combet}, C. and {Crill}, B.~P. and {de Bernardis}, P. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Falgarone}, E. and {Fantaye}, Y. and {Ferri{\`e}re}, K. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Guillet}, V. and {Handley}, W. and {Hansen}, F.~K. and {Herranz}, D. and {Huang}, Z. and {Jaffe}, A.~H. and {Jones}, W.~C. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lamarre}, J. -M. and {Lasenby}, A. and {Le Jeune}, M. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Natoli}, P. and {Pagano}, L. and {Paoletti}, D. and {Pettorino}, V. and {Piacentini}, F. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Rosset}, C. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Soler}, J.~D. and {Spencer}, L.~D. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valiviita}, J. and {Vansyngel}, F. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wehus}, I.~K. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. XI. Polarized dust foregrounds}",
      journal = {AA},
     keywords = {dust, extinction, ISM: magnetic fields, ISM: structure, cosmic background radiation, polarization, submillimeter: diffuse background, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A11},
        pages = {A11},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{LP16,
       author = {{Lazarian}, A. and {Pogosyan}, D.},
        title = "{Spectrum and Anisotropy of Turbulence from Multi-frequency Measurement of Synchrotron Polarization}",
      journal = {ApJ},
     keywords = {ISM: general, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = feb,
       volume = {818},
       number = {2},
          eid = {178},
        pages = {178},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{MO07,
       author = {{McKee}, Christopher F. and {Ostriker}, Eve C.},
        title = "{Theory of Star Formation}",
      journal = {ARAA},
     keywords = {Astrophysics},
         year = 2007,
        month = sep,
       volume = {45},
       number = {1},
        pages = {565-687},
          doi = {10.1146/annurev.astro.45.051806.110602},
archivePrefix = {arXiv},
       eprint = {arXiv:0707.3514},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ARA&A..45..565M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maio97,
       author = {{Maiolino}, R. and {Ruiz}, M. and {Rieke}, G.~H. and {Papadopoulos}, P.},
        title = "{Molecular Gas, Morphology, and Seyfert Galaxy Activity}",
      journal = {ApJ},
     keywords = {Galaxies: Active, Galaxies: ISM, Galaxies: Seyfert, Galaxies: Structure},
         year = 1997,
        month = aug,
       volume = {485},
       number = {2},
        pages = {552-569},
          doi = {10.1086/304438},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...485..552M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{Heck89,
       author = {{Heckman}, T.~M.},
        title = "{CO in Seyfert Galaxies}",
    booktitle = {Active Galactic Nuclei},
         year = 1989,
       editor = {{Osterbrock}, Donald E. and {Miller}, Joseph S.},
       volume = {134},
        month = jan,
        pages = {359},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989IAUS..134..359H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022ApJS..258...10L,
       author = {{Lee}, Janice C. and {Whitmore}, Bradley C. and {Thilker}, David A. and {Deger}, Sinan and {Larson}, Kirsten L. and {Ubeda}, Leonardo and {Anand}, Gagandeep S. and {Boquien}, M{\'e}d{\'e}ric and {Chandar}, Rupali and {Dale}, Daniel A. and {Emsellem}, Eric and {Leroy}, Adam K. and {Rosolowsky}, Erik and {Schinnerer}, Eva and {Schmidt}, Judy and {Lilly}, James and {Turner}, Jordan and {Van Dyk}, Schuyler and {White}, Richard L. and {Barnes}, Ashley T. and {Belfiore}, Francesco and {Bigiel}, Frank and {Blanc}, Guillermo A. and {Cao}, Yixian and {Chevance}, Melanie and {Congiu}, Enrico and {Egorov}, Oleg V. and {Glover}, Simon C.~O. and {Grasha}, Kathryn and {Groves}, Brent and {Henshaw}, Jonathan D. and {Hughes}, Annie and {Klessen}, Ralf S. and {Koch}, Eric and {Kreckel}, Kathryn and {Kruijssen}, J.~M. Diederik and {Liu}, Daizhong and {Lopez}, Laura A. and {Mayker}, Ness and {Meidt}, Sharon E. and {Murphy}, Eric J. and {Pan}, Hsi-An and {Pety}, J{\'e}r{\^o}me and {Querejeta}, Miguel and {Razza}, Alessandro and {Saito}, Toshiki and {S{\'a}nchez-Bl{\'a}zquez}, Patricia and {Santoro}, Francesco and {Sardone}, Amy and {Scheuermann}, Fabian and {Schruba}, Andreas and {Sun}, Jiayi and {Usero}, Antonio and {Watkins}, E. and {Williams}, Thomas G.},
        title = "{The PHANGS-HST Survey: Physics at High Angular Resolution in Nearby Galaxies with the Hubble Space Telescope}",
      journal = {ApJs},
     keywords = {1569, 1567, 1833, 1671, 1560, 761, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jan,
       volume = {258},
       number = {1},
          eid = {10},
        pages = {10},
          doi = {10.3847/1538-4365/ac1fe5},
archivePrefix = {arXiv},
       eprint = {arXiv:2101.02855},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022ApJS..258...10L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{2005AAS...206.1307M,
       author = {{Mutchler}, M. and {Beckwith}, S.~V.~W. and {Bond}, H. and {Christian}, C. and {Frattare}, L. and {Hamilton}, F. and {Hamilton}, M. and {Levay}, Z. and {Noll}, K. and {Royle}, T.},
        title = "{Hubble Space Telescope multi-color ACS mosaic of M51, the Whirlpool Galaxy}",
    booktitle = {American Astronomical Society Meeting Abstracts \#206},
         year = 2005,
       series = {American Astronomical Society Meeting Abstracts},
       volume = {206},
        month = may,
          eid = {13.07},
        pages = {13.07},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005AAS...206.1307M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{M51,
       author = {{Borlaff}, Alejandro S. and {Lopez-Rodriguez}, Enrique and {Beck}, Rainer and {Stepanov}, Rodion and {Ntormousi}, Eva and {Hughes}, Annie and {Tassis}, Konstantinos and {Marcum}, Pamela M. and {Grosset}, Lucas and {Beckman}, John E. and {Proudfit}, Leslie and {Clark}, Susan E. and {D{\'\i}az-Santos}, Tanio and {Mao}, Sui Ann and {Reach}, William T. and {Roman-Duval}, Julia and {Subramanian}, Kandaswamy and {Tram}, Le Ngoc and {Zweibel}, Ellen G. and {Dale}, Daniel and {Legacy Team}},
        title = "{Extragalactic Magnetism with SOFIA (Legacy Program). I. The Magnetic Field in the Multiphase Interstellar Medium of M51}",
      journal = {ApJ},
     keywords = {Spiral galaxies, Extragalactic magnetic fields, Magnetic fields, Star formation, Molecular clouds, Far infrared astronomy, Radio astronomy, Polarimetry, 1560, 507, 994, 1569, 1072, 529, 1338, 1278, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = nov,
       volume = {921},
       number = {2},
          eid = {128},
        pages = {128},
          doi = {10.3847/1538-4357/ac16d7},
archivePrefix = {arXiv},
       eprint = {arXiv:2105.09315},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...921..128B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021ApJ...915...67H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Xu}, Siyao},
        title = "{Anisotropic Turbulence in Position-Position-Velocity Space: Probing Three-dimensional Magnetic Fields}",
      journal = {ApJ},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jul,
       volume = {915},
       number = {1},
          eid = {67},
        pages = {67},
          doi = {10.3847/1538-4357/ac00ab},
archivePrefix = {arXiv},
       eprint = {arXiv:2104.02842},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...915...67H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019A&A...624A..80N,
       author = {{Nersesian}, A. and {Xilouris}, E.~M. and {Bianchi}, S. and {Galliano}, F. and {Jones}, A.~P. and {Baes}, M. and {Casasola}, V. and {Cassar{\`a}}, L.~P. and {Clark}, C.~J.~R. and {Davies}, J.~I. and {Decleir}, M. and {Dobbels}, W. and {De Looze}, I. and {De Vis}, P. and {Fritz}, J. and {Galametz}, M. and {Madden}, S.~C. and {Mosenkov}, A.~V. and {Tr{\v{c}}ka}, A. and {Verstocken}, S. and {Viaene}, S. and {Lianou}, S.},
        title = "{Old and young stellar populations in DustPedia galaxies and their role in dust heating}",
      journal = {AA},
     keywords = {dust, extinction, infrared: galaxies, galaxies: photometry, galaxies: ISM, galaxies: evolution, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {624},
          eid = {A80},
        pages = {A80},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...624A..80N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{2019tuma.book.....B,
       author = {{Beresnyak}, Andrey and {Lazarian}, Alexander},
        title = "{Turbulence in Magnetohydrodynamics}",
         year = 2019,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019tuma.book.....B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019ApJS..244...24L,
       author = {{Leroy}, Adam K. and {Sandstrom}, Karin M. and {Lang}, Dustin and {Lewis}, Alexia and {Salim}, Samir and {Behrens}, Erica A. and {Chastenet}, J{\'e}r{\'e}my and {Chiang}, I-Da and {Gallagher}, Molly J. and {Kessler}, Sarah and {Utomo}, Dyas},
        title = "{A z = 0 Multiwavelength Galaxy Synthesis. I. A WISE and GALEX Atlas of Local Galaxies}",
      journal = {ApJS},
     keywords = {galaxies: general, galaxies: ISM, galaxies: spiral, galaxies: star formation, infrared: galaxies, ultraviolet: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {244},
       number = {2},
          eid = {24},
        pages = {24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..244...24L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2017PASJ...69...18T,
       author = {{Tosaki}, Tomoka and {Kohno}, Kotaro and {Harada}, Nanase and {Tanaka}, Kunihiko and {Egusa}, Fumi and {Izumi}, Takuma and {Takano}, Shuro and {Nakajima}, Taku and {Taniguchi}, Akio and {Tamura}, Yoichi},
        title = "{A statistical study of giant molecular clouds traced by $^{13}$CO, C$^{18}$O, CS, and CH$_{3}$OH in the disk of NGC 1068 based on ALMA observations}",
      journal = {PASJ},
     keywords = {galaxies: individual (NGC 1068), galaxies: ISM, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = apr,
       volume = {69},
       number = {2},
          eid = {18},
        pages = {18},
          doi = {10.1093/pasj/psw122},
archivePrefix = {arXiv},
       eprint = {arXiv:1612.00948},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017PASJ...69...18T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INCOLLECTION{2013pss5.book..641B,
       author = {{Beck}, Rainer and {Wielebinski}, Richard},
        title = "{Magnetic Fields in Galaxies}",
     keywords = {Physics},
    booktitle = {Planets, Stars and Stellar Systems. Volume 5: Galactic Structure and Stellar Populations},
         year = 2013,
       editor = {{Oswalt}, Terry D. and {Gilmore}, Gerard},
       volume = {5},
        pages = {641},
          doi = {10.1007/978-94-007-5612-0\_13},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013pss5.book..641B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021ApJ...912....2H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Stanimirovi{\'c}}, Sne{\v{z}}ana},
        title = "{Revealing Gravitational Collapse in the Serpens G3-G6 Molecular Cloud Using Velocity Gradients}",
      journal = {ApJ},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, Star-forming regions, 847, 845, 839, 1565, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {912},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.3847/1538-4357/abedb7},
archivePrefix = {arXiv},
       eprint = {arXiv:2102.06225},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...912....2H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020NatAs...4..704A,
       author = {{Abbate}, Federico and {Possenti}, Andrea and {Tiburzi}, Caterina and {Barr}, Ewan and {van Straten}, Willem and {Ridolfi}, Alessandro and {Freire}, Paulo},
        title = "{Constraints on the magnetic field in the Galactic halo from globular cluster pulsars}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = mar,
       volume = {4},
        pages = {704-710},
          doi = {10.1038/s41550-020-1030-6},
archivePrefix = {arXiv},
       eprint = {arXiv:2003.02867},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020NatAs...4..704A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2015ARA&A..53..501A,
       author = {{Andersson}, B. -G. and {Lazarian}, A. and {Vaillancourt}, John E.},
        title = "{Interstellar Dust Grain Alignment}",
      journal = {ARAA},
         year = 2015,
        month = aug,
       volume = {53},
        pages = {501-539},
          doi = {10.1146/annurev-astro-082214-122414},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ARA&A..53..501A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2007ApJ...669L..77L,
       author = {{Lazarian}, A. and {Hoang}, Thiem},
        title = "{Subsonic Mechanical Alignment of Irregular Grains}",
      journal = {ApJL},
     keywords = {ISM: Dust, Extinction, ISM: Magnetic Fields, Polarization, Astrophysics},
         year = 2007,
        month = nov,
       volume = {669},
       number = {2},
        pages = {L77-L80},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007ApJ...669L..77L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...888...96H,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Predictions of Cosmic Microwave Background Foreground Dust Polarization Using Velocity Gradients}",
      journal = {ApJ},
     keywords = {845, 847, 322, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/ab60a5},
archivePrefix = {arXiv},
       eprint = {arXiv:1910.05637},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...96H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2021ApJS..255...19L,
       author = {{Leroy}, Adam K. and {Hughes}, Annie and {Liu}, Daizhong and {Pety}, J{\'e}r{\^o}me and {Rosolowsky}, Erik and {Saito}, Toshiki and {Schinnerer}, Eva and {Schruba}, Andreas and {Usero}, Antonio and {Faesi}, Christopher M. and {Herrera}, Cinthya N. and {Chevance}, M{\'e}lanie and {Hygate}, Alexander P.~S. and {Kepley}, Amanda A. and {Koch}, Eric W. and {Querejeta}, Miguel and {Sliwa}, Kazimierz and {Will}, David and {Wilson}, Christine D. and {Anand}, Gagandeep S. and {Barnes}, Ashley and {Belfiore}, Francesco and {Be{\v{s}}li{\'c}}, Ivana and {Bigiel}, Frank and {Blanc}, Guillermo A. and {Bolatto}, Alberto D. and {Boquien}, M{\`e}d{\`e}ric and {Cao}, Yixian and {Chandar}, Rupali and {Chastenet}, J{\'e}r{\'e}my and {Chiang}, I. -Da and {Congiu}, Enrico and {Dale}, Daniel A. and {Deger}, Sinan and {den Brok}, Jakob S. and {Eibensteiner}, Cosima and {Emsellem}, Eric and {Garc{\'\i}a-Rodr{\'\i}guez}, Axel and {Glover}, Simon C.~O. and {Grasha}, Kathryn and {Groves}, Brent and {Henshaw}, Jonathan D. and {Jim{\'e}nez Donaire}, Mar{\'\i}a J. and {Kim}, Jaeyeon and {Klessen}, Ralf S. and {Kreckel}, Kathryn and {Kruijssen}, J.~M. Diederik and {Larson}, Kirsten L. and {Lee}, Janice C. and {Mayker}, Ness and {McElroy}, Rebecca and {Meidt}, Sharon E. and {Mok}, Angus and {Pan}, Hsi-An and {Puschnig}, Johannes and {Razza}, Alessandro and {S{\'a}nchez-Bl'azquez}, Patricia and {Sandstrom}, Karin M. and {Santoro}, Francesco and {Sardone}, Amy and {Scheuermann}, Fabian and {Sun}, Jiayi and {Thilker}, David A. and {Turner}, Jordan A. and {Ubeda}, Leonardo and {Utomo}, Dyas and {Watkins}, Elizabeth J. and {Williams}, Thomas G.},
        title = "{PHANGS-ALMA Data Processing and Pipeline}",
      journal = {ApJs},
     keywords = {Radio interferometry, Interstellar medium, CO line emission, Millimeter astronomy, Astronomy data reduction, Galaxies, Star formation, 1346, 847, 262, 1061, 1861, 573, 1569, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jul,
       volume = {255},
       number = {1},
          eid = {19},
        pages = {19},
          doi = {10.3847/1538-4365/abec80},
archivePrefix = {arXiv},
       eprint = {arXiv:2104.07665},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..255...19L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2020A&A...641A...4P,
       author = {{Planck Collaboration} and {Akrami}, Y. and {Ashdown}, M. and {Aumont}, J. and {Baccigalupi}, C. and {Ballardini}, M. and {Banday}, A.~J. and {Barreiro}, R.~B. and {Bartolo}, N. and {Basak}, S. and {Benabed}, K. and {Bersanelli}, M. and {Bielewicz}, P. and {Bond}, J.~R. and {Borrill}, J. and {Bouchet}, F.~R. and {Boulanger}, F. and {Bucher}, M. and {Burigana}, C. and {Calabrese}, E. and {Cardoso}, J. -F. and {Carron}, J. and {Casaponsa}, B. and {Challinor}, A. and {Colombo}, L.~P.~L. and {Combet}, C. and {Crill}, B.~P. and {Cuttaia}, F. and {de Bernardis}, P. and {de Rosa}, A. and {de Zotti}, G. and {Delabrouille}, J. and {Delouis}, J. -M. and {Di Valentino}, E. and {Dickinson}, C. and {Diego}, J.~M. and {Donzelli}, S. and {Dor{\'e}}, O. and {Ducout}, A. and {Dupac}, X. and {Efstathiou}, G. and {Elsner}, F. and {En{\ss}lin}, T.~A. and {Eriksen}, H.~K. and {Falgarone}, E. and {Fernandez-Cobos}, R. and {Finelli}, F. and {Forastieri}, F. and {Frailis}, M. and {Fraisse}, A.~A. and {Franceschi}, E. and {Frolov}, A. and {Galeotta}, S. and {Galli}, S. and {Ganga}, K. and {G{\'e}nova-Santos}, R.~T. and {Gerbino}, M. and {Ghosh}, T. and {Gonz{\'a}lez-Nuevo}, J. and {G{\'o}rski}, K.~M. and {Gratton}, S. and {Gruppuso}, A. and {Gudmundsson}, J.~E. and {Handley}, W. and {Hansen}, F.~K. and {Helou}, G. and {Herranz}, D. and {Hildebrandt}, S.~R. and {Huang}, Z. and {Jaffe}, A.~H. and {Karakci}, A. and {Keih{\"a}nen}, E. and {Keskitalo}, R. and {Kiiveri}, K. and {Kim}, J. and {Kisner}, T.~S. and {Krachmalnicoff}, N. and {Kunz}, M. and {Kurki-Suonio}, H. and {Lagache}, G. and {Lamarre}, J. -M. and {Lasenby}, A. and {Lattanzi}, M. and {Lawrence}, C.~R. and {Le Jeune}, M. and {Levrier}, F. and {Liguori}, M. and {Lilje}, P.~B. and {Lindholm}, V. and {L{\'o}pez-Caniego}, M. and {Lubin}, P.~M. and {Ma}, Y. -Z. and {Mac{\'\i}as-P{\'e}rez}, J.~F. and {Maggio}, G. and {Maino}, D. and {Mandolesi}, N. and {Mangilli}, A. and {Marcos-Caballero}, A. and {Maris}, M. and {Martin}, P.~G. and {Mart{\'\i}nez-Gonz{\'a}lez}, E. and {Matarrese}, S. and {Mauri}, N. and {McEwen}, J.~D. and {Meinhold}, P.~R. and {Melchiorri}, A. and {Mennella}, A. and {Migliaccio}, M. and {Miville-Desch{\^e}nes}, M. -A. and {Molinari}, D. and {Moneti}, A. and {Montier}, L. and {Morgante}, G. and {Natoli}, P. and {Oppizzi}, F. and {Pagano}, L. and {Paoletti}, D. and {Partridge}, B. and {Peel}, M. and {Pettorino}, V. and {Piacentini}, F. and {Polenta}, G. and {Puget}, J. -L. and {Rachen}, J.~P. and {Reinecke}, M. and {Remazeilles}, M. and {Renzi}, A. and {Rocha}, G. and {Roudier}, G. and {Rubi{\~n}o-Mart{\'\i}n}, J.~A. and {Ruiz-Granados}, B. and {Salvati}, L. and {Sandri}, M. and {Savelainen}, M. and {Scott}, D. and {Seljebotn}, D.~S. and {Sirignano}, C. and {Spencer}, L.~D. and {Suur-Uski}, A. -S. and {Tauber}, J.~A. and {Tavagnacco}, D. and {Tenti}, M. and {Thommesen}, H. and {Toffolatti}, L. and {Tomasi}, M. and {Trombetti}, T. and {Valiviita}, J. and {Van Tent}, B. and {Vielva}, P. and {Villa}, F. and {Vittorio}, N. and {Wandelt}, B.~D. and {Wehus}, I.~K. and {Zacchei}, A. and {Zonca}, A.},
        title = "{Planck 2018 results. IV. Diffuse component separation}",
      journal = {AA},
     keywords = {ISM: general, cosmology: observations, cosmic background radiation, diffuse radiation, Galaxy: general, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = sep,
       volume = {641},
          eid = {A4},
        pages = {A4},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020A&A...641A...4P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011MNRAS.412.2396F,
       author = {{Fletcher}, A. and {Beck}, R. and {Shukurov}, A. and {Berkhuijsen}, E.~M. and {Horellou}, C.},
        title = "{Magnetic fields and spiral arms in the galaxy M51}",
      journal = {MNRAS},
     keywords = {galaxies: individual: M51, galaxies: ISM, galaxies: magnetic fields, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = apr,
       volume = {412},
       number = {4},
        pages = {2396-2416},
          doi = {10.1111/j.1365-2966.2010.18065.x},
archivePrefix = {arXiv},
       eprint = {arXiv:1001.5230},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.412.2396F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2013MNRAS.433.1675B,
       author = {{Basu}, Aritra and {Roy}, Subhashis},
        title = "{Magnetic fields in nearby normal galaxies: energy equipartition}",
      journal = {MNRAS},
     keywords = {cosmic rays, ISM: general, galaxies: ISM, galaxies: magnetic fields, galaxies: spiral, radio continuum: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = aug,
       volume = {433},
       number = {2},
        pages = {1675-1686},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.433.1675B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{2017A&A...597A..85B,
       author = {{Beuther}, H. and {Meidt}, S. and {Schinnerer}, E. and {Paladino}, R. and {Leroy}, A.},
        title = "{Interactions of the Galactic bar and spiral arm in NGC 3627}",
      journal = {AA},
     keywords = {stars: formation, galaxies: individual: NGC 3627, stars: massive, ISM: clouds, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A85},
        pages = {A85},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A..85B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003A&A...407..485G,
       author = {{Garc{\'\i}a-Burillo}, S. and {Combes}, F. and {Hunt}, L.~K. and {Boone}, F. and {Baker}, A.~J. and {Tacconi}, L.~J. and {Eckart}, A. and {Neri}, R. and {Leon}, S. and {Schinnerer}, E. and {Englmaier}, P.},
        title = "{Molecular Gas in NUclei of GAlaxies (NUGA). I. The counter-rotating LINER NGC 4826}",
      journal = {AA},
     keywords = {galaxies: individual: NGC 4826, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, radio lines: galaxies, Astrophysics},
         year = 2003,
        month = aug,
       volume = {407},
        pages = {485-502},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...407..485G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2005A&A...444..739B,
       author = {{Beck}, R. and {Fletcher}, A. and {Shukurov}, A. and {Snodin}, A. and {Sokoloff}, D.~D. and {Ehle}, M. and {Moss}, D. and {Shoutenkov}, V.},
        title = "{Magnetic fields in barred galaxies. IV. NGC 1097 and NGC 1365}",
      journal = {AA},
     keywords = {galaxies: magnetic fields, galaxies:, individual: NGC 1097, NGC 1365, galaxies: spiral, galaxies: structure, ISM: magnetic fields, galaxies: nuclei, Astrophysics},
         year = 2005,
        month = dec,
       volume = {444},
       number = {3},
        pages = {739-765},
          doi = {10.1051/0004-6361:20053556},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508485},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...444..739B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021ApJ...912L..27E,
       author = {{Eswaraiah}, Chakali and {Li}, Di and {Furuya}, Ray S. and {Hasegawa}, Tetsuo and {Ward-Thompson}, Derek and {Qiu}, Keping and {Ohashi}, Nagayoshi and {Pattle}, Kate and {Sadavoy}, Sarah and {Hull}, Charles L.~H. and {Berry}, David and {Doi}, Yasuo and {Ching}, Tao-Chung and {Lai}, Shih-Ping and {Wang}, Jia-Wei and {Koch}, Patrick M. and {Kwon}, Jungmi and {Kwon}, Woojin and {Bastien}, Pierre and {Arzoumanian}, Doris and {Coud{\'e}}, Simon and {Soam}, Archana and {Fanciullo}, Lapo and {Yen}, Hsi-Wei and {Liu}, Junhao and {Hoang}, Thiem and {Ping Chen}, Wen and {Shimajiri}, Yoshito and {Liu}, Tie and {Chen}, Zhiwei and {Li}, Hua-bai and {Lyo}, A. -Ran and {Hwang}, Jihye and {Johnstone}, Doug and {Rao}, Ramprasad and {Bich Ngoc}, Nguyen and {Ngoc Diep}, Pham and {Mairs}, Steve and {Parsons}, Harriet and {Tamura}, Motohide and {Tahani}, Mehrnoosh and {Vivien Chen}, Huei-Ru and {Nakamura}, Fumitaka and {Shinnaga}, Hiroko and {Tang}, Ya-Wen and {Cho}, Jungyeon and {Won Lee}, Chang and {Inutsuka}, Shu-ichiro and {Inoue}, Tsuyoshi and {Iwasaki}, Kazunari and {Qian}, Lei and {Xie}, Jinjin and {Li}, Dalei and {Liu}, Hong-Li and {Zhang}, Chuan-Peng and {Chen}, Mike and {Zhang}, Guoyin and {Zhu}, Lei and {Zhou}, Jianjun and {Andr{\'e}}, Philippe and {Liu}, Sheng-Yuan and {Yuan}, Jinghua and {Lu}, Xing and {Peretto}, Nicolas and {Bourke}, Tyler L. and {Byun}, Do-Young and {Dai}, Sophia and {Duan}, Yan and {Duan}, Hao-Yuan and {Eden}, David and {Matthews}, Brenda and {Fiege}, Jason and {Fissel}, Laura M. and {Kim}, Kee-Tae and {Lee}, Chin-Fei and {Kim}, Jongsoo and {Pyo}, Tae-Soo and {Choi}, Yunhee and {Choi}, Minho and {Chrysostomou}, Antonio and {Jung Chung}, Eun and {Ngoc Tram}, Le and {Franzmann}, Erica and {Friberg}, Per and {Friesen}, Rachel and {Fuller}, Gary and {Gledhill}, Tim and {Graves}, Sarah and {Greaves}, Jane and {Griffin}, Matt and {Gu}, Qilao and {Han}, Ilseung and {Hatchell}, Jennifer and {Hayashi}, Saeko and {Houde}, Martin and {Kawabata}, Koji and {Jeong}, Il-Gyo and {Kang}, Ji-hyun and {Kang}, Sung-ju and {Kang}, Miju and {Kataoka}, Akimasa and {Kemper}, Francisca and {Rawlings}, Mark and {Rawlings}, Jonathan and {Retter}, Brendan and {Richer}, John and {Rigby}, Andrew and {Saito}, Hiro and {Savini}, Giorgio and {Scaife}, Anna and {Seta}, Masumichi and {Kim}, Gwanjeong and {Hee Kim}, Kyoung and {Kim}, Mi-Ryang and {Kirchschlager}, Florian and {Kirk}, Jason and {Kobayashi}, Masato I.~N. and {Konyves}, Vera and {Kusune}, Takayoshi and {Lacaille}, Kevin and {Law}, Chi-Yan and {Lee}, Sang-Sung and {Lee}, Yong-Hee and {Matsumura}, Masafumi and {Moriarty-Schieven}, Gerald and {Nagata}, Tetsuya and {Nakanishi}, Hiroyuki and {Onaka}, Takashi and {Park}, Geumsook and {Tang}, Xindi and {Tomisaka}, Kohji and {Tsukamoto}, Yusuke and {Viti}, Serena and {Wang}, Hongchi and {Whitworth}, Anthony and {Yoo}, Hyunju and {Yun}, Hyeong-Sik and {Zenko}, Tetsuya and {Zhang}, Yapeng and {de Looze}, Ilse and {Dowell}, C. Darren and {Eyres}, Stewart and {Falle}, Sam and {Robitaille}, Jean-Fran{\c{c}}ois and {van Loo}, Sven},
        title = "{The JCMT BISTRO Survey: Revealing the Diverse Magnetic Field Morphologies in Taurus Dense Cores with Sensitive Submillimeter Polarimetry}",
      journal = {ApJL},
     keywords = {Dust continuum emission, Polarimetry, Low mass stars, Dense interstellar clouds, Interstellar magnetic fields, 412, 1278, 2050, 371, 845, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = may,
       volume = {912},
       number = {2},
          eid = {L27},
        pages = {L27},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...912L..27E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021arXiv210407739L,
       author = {{Leroy}, Adam K. and {Schinnerer}, Eva and {Hughes}, Annie and {Rosolowsky}, Erik and {Pety}, J{\'e}r{\^o}me and {Schruba}, Andreas and {Usero}, Antonio and {Blanc}, Guillermo A. and {Chevance}, M{\'e}lanie and {Emsellem}, Eric and {Faesi}, Christopher M. and {Herrera}, Cinthya N. and {Liu}, Daizhong and {Meidt}, Sharon E. and {Querejeta}, Miguel and {Saito}, Toshiki and {Sandstrom}, Karin M. and {Sun}, Jiayi and {Williams}, Thomas G. and {Anand}, Gagandeep S. and {Barnes}, Ashley T. and {Behrens}, Erica A. and {Belfiore}, Francesco and {Benincasa}, Samantha M. and {Be{\v{s}}li{\'c}}, Ivana and {Bigiel}, Frank and {Bolatto}, Alberto D. and {den Brok}, Jakob S. and {Cao}, Yixian and {Chandar}, Rupali and {Chastenet}, J{\'e}r{\'e}my and {Chiang}, I. -Da and {Congiu}, Enrico and {Dale}, Daniel A. and {Deger}, Sinan and {Eibensteiner}, Cosima and {Egorov}, Oleg V. and {Garc{\'\i}a-Rodr{\'\i}guez}, Axel and {Glover}, Simon C.~O. and {Grasha}, Kathryn and {Henshaw}, Jonathan D. and {Ho}, I. -Ting and {Kepley}, Amanda A. and {Kim}, Jaeyeon and {Klessen}, Ralf S. and {Kreckel}, Kathryn and {Koch}, Eric W. and {Kruijssen}, J.~M. Diederik and {Larson}, Kirsten L. and {Lee}, Janice C. and {Lopez}, Laura A. and {Machado}, Josh and {Mayker}, Ness and {McElroy}, Rebecca and {Murphy}, Eric J. and {Ostriker}, Eve C. and {Pan}, Hsi-An and {Pessa}, Ismael and {Puschnig}, Johannes and {Razza}, Alessandro and {S{\'a}nchez-Bl{\'a}zquez}, Patricia and {Santoro}, Francesco and {Sardone}, Amy and {Scheuermann}, Fabian and {Sliwa}, Kazimierz and {Sormani}, Mattia C. and {Stuber}, Sophia K. and {Thilker}, David A. and {Turner}, Jordan A. and {Utomo}, Dyas and {Watkins}, Elizabeth J. and {Whitmore}, Bradley},
        title = "{PHANGS-ALMA: Arcsecond CO(2-1) Imaging of Nearby Star-forming Galaxies}",
      journal = {ApJs},
     keywords = {847, 653, 1560, 1061, 594, 262, 136, 391, 573, 1569, 1338, 1602, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = dec,
       volume = {257},
       number = {2},
          eid = {43},
        pages = {43},
          doi = {10.3847/1538-4365/ac17f3},
archivePrefix = {arXiv},
       eprint = {arXiv:2104.07739},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..257...43L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...779...46H,
       author = {{Hughes}, Annie and {Meidt}, Sharon E. and {Colombo}, Dario and {Schinnerer}, Eva and {Pety}, Jer{\^o}me and {Leroy}, Adam K. and {Dobbs}, Clare L. and {Garc{\'\i}a-Burillo}, Santiago and {Thompson}, Todd A. and {Dumas}, Ga{\"e}lle and {Schuster}, Karl F. and {Kramer}, Carsten},
        title = "{A Comparative Study of Giant Molecular Clouds in M51, M33, and the Large Magellanic Cloud}",
      journal = {ApJ},
     keywords = {galaxies: individual: M51 M33 Large Magellanic Cloud, galaxies: ISM, ISM: clouds, ISM: molecules, ISM: structure, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2013,
        month = dec,
       volume = {779},
       number = {1},
          eid = {46},
        pages = {46},
          doi = {10.1088/0004-637X/779/1/46},
archivePrefix = {arXiv},
       eprint = {arXiv:1309.3453},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...779...46H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2018JAI.....740008H,
       author = {{Harper}, Doyal A. and {Runyan}, Marcus C. and {Dowell}, C. Darren and {Wirth}, C. Jesse and {Amato}, Michael and {Ames}, Troy and {Amiri}, Mandana and {Banks}, Stuart and {Bartels}, Arlin and {Benford}, Dominic J. and {Berthoud}, Marc and {Buchanan}, Ernest and {Casey}, Sean and {Chapman}, Nicholas L. and {Chuss}, David T. and {Cook}, Brant and {Derro}, Rebecca and {Dotson}, Jessie L. and {Evans}, Rhodri and {Fixsen}, Dale and {Gatley}, Ian and {Guerra}, Jordan A. and {Halpern}, Mark and {Hamilton}, Ryan T. and {Hamlin}, Louise A. and {Hansen}, Christopher J. and {Heimsath}, Stephen and {Hermida}, Alfonso and {Hilton}, Gene C. and {Hirsch}, Robert and {Hollister}, Matthew I. and {Hostetter}, Carl F. and {Irwin}, Kent and {Jhabvala}, Christine A. and {Jhabvala}, Murzban and {Kastner}, Joel and {Kov{\'a}cs}, Attila and {Lin}, Sean and {Loewenstein}, Robert F. and {Looney}, Leslie W. and {Lopez-Rodriguez}, Enrique and {Maher}, Stephen F. and {Michail}, Joseph M. and {Miller}, Timothy M. and {Moseley}, S. Harvey and {Novak}, Giles and {Pernic}, Robert J. and {Rennick}, Timothy and {Rhody}, Harvey and {Sandberg}, Eric and {Sandford}, Dale and {Santos}, Fabio Pereira and {Shafer}, Rick and {Sharp}, Elmer H. and {Shirron}, Peter and {Siah}, Javad and {Silverberg}, Robert and {Sparr}, Leroy M. and {Spotz}, Robert and {Staguhn}, Johannes G. and {Toorian}, Armen S. and {Towey}, Shannon and {Tuttle}, Jim and {Vaillancourt}, John and {Voellmer}, George and {Volpert}, Carolyn G. and {Wang}, Shu-I. and {Wollack}, Edward J.},
        title = "{HAWC+, the Far-Infrared Camera and Polarimeter for SOFIA}",
      journal = {Journal of Astronomical Instrumentation},
     keywords = {Instrumentation, polarimeters, camera, far-infrared, detectors, stars, formation, dust},
         year = 2018,
        month = jan,
       volume = {7},
       number = {4},
          eid = {1840008-1025},
        pages = {1840008-1025},
          doi = {10.1142/S2251171718400081},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018JAI.....740008H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2001ApJ...554.1175M,
       author = {{Maron}, Jason and {Goldreich}, Peter},
        title = "{Simulations of Incompressible Magnetohydrodynamic Turbulence}",
      journal = {ApJ},
     keywords = {Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2001,
        month = jun,
       volume = {554},
       number = {2},
        pages = {1175-1196},
          doi = {10.1086/321413},
archivePrefix = {arXiv},
       eprint = {astro-ph/0012491},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...554.1175M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2000A&A...355..128C,
       author = {{Chy{\.z}y}, K.~T. and {Beck}, R. and {Kohle}, S. and {Klein}, U. and {Urbanik}, M.},
        title = "{Regular magnetic fields in the dwarf irregular galaxy NGC 4449}",
      journal = {AA},
     keywords = {GALAXIES: MAGNETIC FIELDS, GALAXIES: IRREGULAR, GALAXIES: INDIVIDUAL:, RADIO CONTINUUM: GALAXIES, POLARIZATION, Astrophysics},
         year = 2000,
        month = mar,
       volume = {355},
        pages = {128-137},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...355..128C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1960StoAn..21....3L,
       author = {{Lindblad}, Per Olof},
        title = "{On tidal interaction between galaxies}",
      journal = {Stockholms Observatoriums Annaler},
     keywords = {CELESTIAL MECHANICS, GALAXIES},
         year = 1960,
        month = jan,
       volume = {3},
        pages = {3},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1960StoAn..21....3L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1964ApJ...140..646L,
       author = {{Lin}, C.~C. and {Shu}, Frank H.},
        title = "{On the Spiral Structure of Disk Galaxies.}",
      journal = {ApJ},
         year = 1964,
        month = aug,
       volume = {140},
        pages = {646},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1964ApJ...140..646L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...550..752V,
       author = {{Vishniac}, Ethan T. and {Cho}, Jungyeon},
        title = "{Magnetic Helicity Conservation and Astrophysical Dynamos}",
      journal = {ApJ},
     keywords = {ISM: Magnetic Fields, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics, Physics - Plasma Physics},
         year = 2001,
        month = apr,
       volume = {550},
       number = {2},
        pages = {752-760},
          doi = {10.1086/319817},
archivePrefix = {arXiv},
       eprint = {astro-ph/0010373},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001ApJ...550..752V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1978A&A....70..367C,
       author = {{Cesarsky}, C.~J. and {Volk}, H.~J.},
        title = "{Cosmic Ray Penetration into Molecular Clouds}",
      journal = {AA},
         year = 1978,
        month = nov,
       volume = {70},
        pages = {367},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978A&A....70..367C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...530A.109P,
       author = {{Padovani}, M. and {Galli}, D.},
        title = "{Effects of magnetic fields on the cosmic-ray ionization of molecular cloud cores}",
      journal = {AA},
     keywords = {cosmic rays, ISM: clouds, ISM: magnetic fields, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = jun,
       volume = {530},
          eid = {A109},
        pages = {A109},
          doi = {10.1051/0004-6361/201116853},
archivePrefix = {arXiv},
       eprint = {arXiv:1104.5445},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...530A.109P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2000ApJ...539..273C,
       author = {{Cho}, Jungyeon and {Vishniac}, Ethan T.},
        title = "{The Anisotropy of Magnetohydrodynamic Alfv{\'e}nic Turbulence}",
      journal = {ApJ},
     keywords = {ISM: General, Magnetic Fields, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2000,
        month = aug,
       volume = {539},
       number = {1},
        pages = {273-282},
          doi = {10.1086/309213},
archivePrefix = {arXiv},
       eprint = {astro-ph/0003403},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...539..273C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{2011MNRAS.412.2396F,
       author = {{Fletcher}, A. and {Beck}, R. and {Shukurov}, A. and {Berkhuijsen}, E.~M. and {Horellou}, C.},
        title = "{Magnetic fields and spiral arms in the galaxy M51}",
      journal = {MNRAS},
     keywords = {galaxies: individual: M51, galaxies: ISM, galaxies: magnetic fields, galaxies: spiral, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2011,
        month = apr,
       volume = {412},
       number = {4},
        pages = {2396-2416},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011MNRAS.412.2396F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...816...15W,
       author = {{Wang}, Xin and {Tu}, Chuanyi and {Marsch}, Eckart and {He}, Jiansen and {Wang}, Linghua},
        title = "{Scale-dependent Normalized Amplitude and Weak Spectral Anisotropy of Magnetic Field Fluctuations in the Solar Wind Turbulence}",
      journal = {ApJ},
     keywords = {magnetic fields, plasmas, solar wind, turbulence},
         year = 2016,
        month = jan,
       volume = {816},
       number = {1},
          eid = {15},
        pages = {15},
          doi = {10.3847/0004-637X/816/1/15},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...816...15W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2002ApJ...564..291C,
       author = {{Cho}, Jungyeon and {Lazarian}, Alex and {Vishniac}, Ethan T.},
        title = "{Simulations of Magnetohydrodynamic Turbulence in a Strongly Magnetized Medium}",
      journal = {ApJ},
     keywords = {ISM: General, Methods: Numerical, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2002,
        month = jan,
       volume = {564},
       number = {1},
        pages = {291-301},
          doi = {10.1086/324186},
archivePrefix = {arXiv},
       eprint = {astro-ph/0105235},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2002ApJ...564..291C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{survey,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, Victor and {Ho}, Ka Wai and {Benjamin}, Robert A. and {Hill}, Alex S. and {Lockman}, Felix J. and {Goldsmith}, Paul F. and {Lazarian}, Alex},
        title = "{Magnetic field morphology in interstellar clouds with the velocity gradient technique}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = jun,
       volume = {3},
        pages = {776-782},
          doi = {10.1038/s41550-019-0769-0},
archivePrefix = {arXiv},
       eprint = {arXiv:2002.09948},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019NatAs...3..776H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2018ApJ...855...72L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho and {Lee}, Hyeseung and {Cho}, J.},
        title = "{Erratum: {\textquotedblleft}Synchrotron Intensity Gradients as Tracers of Interstellar Magnetic Fields{\textquotedblright}}",
      journal = {ApJ},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = mar,
       volume = {855},
       number = {1},
          eid = {72},
        pages = {72},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...855...72L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...865...59L,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Gradients of Synchrotron Polarization: Tracing 3D Distribution of Magnetic Fields}",
      journal = {ApJ},
     keywords = {ISM: general, ISM: magnetic fields, ISM: structure, magnetohydrodynamics: MHD, radio continuum: ISM, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = sep,
       volume = {865},
       number = {1},
          eid = {59},
        pages = {59},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865...59L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021arXiv210709063L,
       author = {{Lopez-Rodriguez}, Enrique and {Beck}, Rainer and {Clark}, Susan E. and {Hughes}, Annie and {Borlaff}, Alejandro S. and {Ntormousi}, Evangelia and {Grosset}, Lucas and {Tassis}, Konstantinos and {Beckman}, John E. and {Subramanian}, Kandaswamy and {Dale}, Daniel and {D{\'\i}az-Santos}, Tanio},
        title = "{Extragalactic Magnetism with SOFIA (Legacy Program) - II: A Magnetically Driven Flow in the Starburst Ring of NGC 1097}",
      journal = {ApJ},
     keywords = {1278, 1447, 507, 136, 2134, 845, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = dec,
       volume = {923},
       number = {2},
          eid = {150},
        pages = {150},
          doi = {10.3847/1538-4357/ac2e01},
archivePrefix = {arXiv},
       eprint = {arXiv:2107.09063},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...923..150L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2001A&A...378...40S,
       author = {{Soida}, M. and {Urbanik}, M. and {Beck}, R. and {Wielebinski}, R. and {Balkowski}, C.},
        title = "{Unusual magnetic fields in the interacting spiral NGC 3627}",
      journal = {AA},
     keywords = {GALAXIES: MAGNETIC FIELDS, GALAXIES: INTERACTING, GALAXIES: INDIVIDUAL: NGC 3627, RADIO CONTINUUM: GALAXIES, Astrophysics},
         year = 2001,
        month = oct,
       volume = {378},
        pages = {40-50},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2001A&A...378...40S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{H2,
       author = {{Hu}, Yue and {Lazarian}, A. and {Bialy}, Shmuel},
        title = "{Study Turbulence and Probe Magnetic Fields Using the Gradient Technique: Application to H I-to-H$_{2}$ Transition Regions}",
      journal = {ApJ},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = dec,
       volume = {905},
       number = {2},
          eid = {129},
        pages = {129},
          doi = {10.3847/1538-4357/abc3c6},
archivePrefix = {arXiv},
       eprint = {arXiv:2008.00387},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...905..129H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020MNRAS.496.2868L,
       author = {{Lu}, Zekun and {Lazarian}, A. and {Pogosyan}, Dmitri},
        title = "{Producing synthetic maps of dust polarization using a velocity channel gradient technique}",
      journal = {MNRAS},
     keywords = {radio lines: ISM, ISM: magnetic fields, polarization, Diffuse radiation, ISM: structure, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = aug,
       volume = {496},
       number = {3},
        pages = {2868-2884},
          doi = {10.1093/mnras/staa1570},
archivePrefix = {arXiv},
       eprint = {arXiv:1910.02226},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.2868L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020ApJ...888...66L,
       author = {{Lopez-Rodriguez}, Enrique and {Dowell}, C. Darren and {Jones}, Terry J. and {Harper}, Doyal A. and {Berthoud}, Marc and {Chuss}, David and {Dale}, Daniel A. and {Guerra}, Jordan A. and {Hamilton}, Ryan T. and {Looney}, Leslie W. and {Michail}, Joseph M. and {Nikutta}, Robert and {Novak}, Giles and {Santos}, Fabio P. and {Sheth}, Kartik and {Siah}, Javad and {Staguhn}, Johannes and {Stephens}, Ian W. and {Tassis}, Konstantinos and {Trinh}, Christopher Q. and {Ward-Thompson}, Derek and {Werner}, Michael and {Wollack}, Edward J. and {Zweibel}, Ellen G. and {HAWC+Science Team}},
        title = "{SOFIA/HAWC+ Traces the Magnetic Fields in NGC 1068}",
      journal = {ApJ},
     keywords = {Active galactic nuclei, Polarimetry, Spiral galaxies, Spiral pitch angle, Far infrared astronomy, 16, 1278, 1560, 1561, 529, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jan,
       volume = {888},
       number = {2},
          eid = {66},
        pages = {66},
          doi = {10.3847/1538-4357/ab5849},
archivePrefix = {arXiv},
       eprint = {arXiv:1907.06648},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...888...66L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992AJ....103..422K,
       author = {{Kaneko}, Noboru and {Satoh}, Tetsuya and {Toyama}, Kiyotaka and {Sasaki}, Minoru and {Nishimura}, Masaki and {Yamamoto}, Masafumi},
        title = "{Observation of the Velocity Curves of NGC 1068}",
      journal = {AJ},
     keywords = {Galactic Rotation, Spiral Galaxies, Starburst Galaxies, Velocity Distribution, Carbon Monoxide, Forbidden Transitions, H Alpha Line, H Beta Line, Nitrogen, Oxygen Spectra, Astrophysics, GALAXIES: STARSBURST, GALAXIES: KINEMATICS AND DYNAMICS},
         year = 1992,
        month = feb,
       volume = {103},
        pages = {422},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992AJ....103..422K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{doublepeak,
       author = {{Hu}, Yue and {Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Velocity Gradient in the Presence of Self-gravity: Identifying Gravity-induced Inflow and Determining Collapsing Stage}",
      journal = {ApJ},
     keywords = {Interstellar magnetic fields, Interstellar medium, Star formation, Star-forming regions, Star forming regions, 845, 1569, 847, 1565, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jul,
       volume = {897},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-4357/ab9948},
archivePrefix = {arXiv},
       eprint = {arXiv:2002.06754},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...897..123H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2013ApJ...762L..27H,
       author = {{Hu}, Tao and {Shao}, Zhengyi and {Peng}, Qiuhe},
        title = "{New Estimates of the Inclination, Position Angle, Pitch Angle, and Scale Height of the Whirlpool Galaxy}",
      journal = {ApJl},
     keywords = {galaxies: individual: M51, galaxies: spiral, galaxies: structure},
         year = 2013,
        month = jan,
       volume = {762},
       number = {2},
          eid = {L27},
        pages = {L27},
          doi = {10.1088/2041-8205/762/2/L27},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...762L..27H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{LV99,
       author = {{Lazarian}, A. and {Vishniac}, Ethan T.},
        title = "{Reconnection in a Weakly Stochastic Field}",
      journal = {ApJ},
     keywords = {GALAXIES: MAGNETIC FIELDS, MAGNETOHYDRODYNAMICS: MHD, Galaxies: Magnetic Fields, Magnetohydrodynamics: MHD, Astrophysics, Physics - Fluid Dynamics, Physics - Geophysics, Physics - Plasma Physics, Physics - Space Physics},
         year = 1999,
        month = jun,
       volume = {517},
       number = {2},
        pages = {700-718},
          doi = {10.1086/307233},
archivePrefix = {arXiv},
       eprint = {astro-ph/9811037},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999ApJ...517..700L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{GS95,
       author = {{Goldreich}, P. and {Sridhar}, S.},
        title = "{Toward a Theory of Interstellar Turbulence. II. Strong Alfvenic Turbulence}",
      journal = {ApJ},
     keywords = {Interstellar Space, Magnetic Fields, Magnetohydrodynamic Turbulence, Magnetohydrodynamic Waves, Electron Density (Concentration), Energy Spectra, Radio Waves, Variations, Wave Scattering, Astrophysics, ISM: GENERAL, MAGNETOHYDRODYNAMICS: MHD, TURBULENCE},
         year = 1995,
        month = jan,
       volume = {438},
        pages = {763},
          doi = {10.1086/175121},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995ApJ...438..763G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{LP00,
       author = {{Lazarian}, A. and {Pogosyan}, D.},
        title = "{Velocity Modification of H I Power Spectrum}",
      journal = {ApJ},
     keywords = {Galaxy: Structure, ISM: Kinematics and Dynamics, Radio Lines: ISM, Astrophysics},
         year = 2000,
        month = jul,
       volume = {537},
       number = {2},
        pages = {720-748},
          doi = {10.1086/309040},
archivePrefix = {arXiv},
       eprint = {astro-ph/9901241},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000ApJ...537..720L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{PCA,
       author = {{Hu}, Yue and {Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Improving the accuracy of magnetic field tracing by velocity gradients: principal component analysis}",
      journal = {MNRAS},
     keywords = {magnetohydrodynamics (MHD), turbulence, methods: numerical, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = oct,
       volume = {480},
       number = {1},
        pages = {1333-1339},
          doi = {10.1093/mnras/sty1807},
archivePrefix = {arXiv},
       eprint = {arXiv:1802.08772},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.480.1333H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1992MNRAS.259..345A,
       author = {{Athanassoula}, E.},
        title = "{The existence and shapes of dust lanes in galactic bars.}",
      journal = {MNRAS},
     keywords = {Barred Galaxies, Cosmic Dust, Galactic Rotation, Gas Flow, Stellar Motions, Astronomical Models, Celestial Mechanics, Astrophysics},
         year = 1992,
        month = nov,
       volume = {259},
        pages = {345-364},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{LY18a,
       author = {{Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Tracing Magnetic Fields with Spectroscopic Channel Maps}",
      journal = {ApJ},
     keywords = {ISM: magnetic fields, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = jan,
       volume = {853},
       number = {1},
          eid = {96},
        pages = {96},
          doi = {10.3847/1538-4357/aaa241},
archivePrefix = {arXiv},
       eprint = {arXiv:1703.03119},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...853...96L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{CMZ,
       author = {{Hu}, Yue and {Lazarian}, A. and {Wang}, Q. Daniel},
        title = "{Multiscale magnetic fields in the central molecular zone: inference from the gradient technique}",
      journal = {MNRAS},
     keywords = {magnetic field, turbulence, ISM:general, ISM:magnetic field, Galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = mar,
       volume = {511},
       number = {1},
        pages = {829-842},
          doi = {10.1093/mnras/stac159},
archivePrefix = {arXiv},
       eprint = {arXiv:2105.03605},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.511..829H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{YL17a,
       author = {{Yuen}, Ka Ho and {Lazarian}, A.},
        title = "{Tracing Interstellar Magnetic Field Using Velocity Gradient Technique: Application to Atomic Hydrogen Data}",
      journal = {ApJl},
     keywords = {ISM: general, ISM: magnetic fields, ISM: structure, magnetohydrodynamics: MHD, radio lines: ISM, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = mar,
       volume = {837},
       number = {2},
          eid = {L24},
        pages = {L24},
          doi = {10.3847/2041-8213/aa6255},
archivePrefix = {arXiv},
       eprint = {arXiv:1701.07944},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...837L..24Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2021arXiv210913670L,
       author = {{Liu}, Mingrui and {Hu}, Yue and {Lazarian}, A.},
        title = "{Velocity gradients: magnetic field tomography towards the supernova remnant W44}",
      journal = {MNRAS},
     keywords = {MHD, turbulence, ISM: general, ISM: magnetic fields, ISM: supernovae remnants, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = mar,
       volume = {510},
       number = {4},
        pages = {4952-4961},
          doi = {10.1093/mnras/stab3783},
archivePrefix = {arXiv},
       eprint = {arXiv:2109.13670},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.510.4952L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2020arXiv200715344A,
       author = {{Alina}, D. and {Montillaud}, J. and {Hu}, Y. and {Lazarian}, A. and {Ristorcelli}, I. and {Abdikamalov}, E. and {Sagynbayeva}, S. and {Juvela}, M. and {Liu}, T. and {Carri{\`e}re}, J. -S.},
        title = "{Large-scale magnetic field in the Monoceros OB 1 east molecular cloud}",
      journal = {AA},
     keywords = {ISM: magnetic fields, ISM: clouds, ISM: general, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = feb,
       volume = {658},
          eid = {A90},
        pages = {A90},
          doi = {10.1051/0004-6361/202039065},
archivePrefix = {arXiv},
       eprint = {arXiv:2007.15344},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...658A..90A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021ApJ...915L...8D,
       author = {{Duan}, Die and {He}, Jiansen and {Bowen}, Trevor A. and {Woodham}, Lloyd D. and {Wang}, Tieyan and {Chen}, Christopher H.~K. and {Mallet}, Alfred and {Bale}, Stuart D.},
        title = "{Anisotropy of Solar Wind Turbulence in the Inner Heliosphere at Kinetic Scales: PSP Observations}",
      journal = {ApJl},
     keywords = {Solar wind, Interplanetary turbulence, Alfven waves, 1534, 830, 23, Physics - Space Physics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = jul,
       volume = {915},
       number = {1},
          eid = {L8},
        pages = {L8},
          doi = {10.3847/2041-8213/ac07ac},
archivePrefix = {arXiv},
       eprint = {arXiv:2102.13294},
 primaryClass = {physics.space-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...915L...8D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020FrASS...7...83M,
       author = {{Matteini}, L. and {Franci}, L. and {Alexandrova}, O. and {Lacombe}, C. and {Landi}, S. and {Hellinger}, P. and {Papini}, E. and {Verdini}, A.},
        title = "{Magnetic field turbulence in the solar wind at sub-ion scales: in situ observations and numerical simulations}",
      journal = {Frontiers in Astronomy and Space Sciences},
     keywords = {Solar wind, Plasma turbulence, Numerical Simulations, In situ observation, Kinetic physics, Physics - Space Physics},
         year = 2020,
        month = dec,
       volume = {7},
          eid = {83},
        pages = {83},
          doi = {10.3389/fspas.2020.563075},
archivePrefix = {arXiv},
       eprint = {arXiv:2008.13219},
 primaryClass = {physics.space-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020FrASS...7...83M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2010ApJ...710..853C,
       author = {{Chepurnov}, A. and {Lazarian}, A.},
        title = "{Extending the Big Power Law in the Sky with Turbulence Spectra from Wisconsin H{\ensuremath{\alpha}} Mapper Data}",
      journal = {ApJ},
     keywords = {ISM: lines and bands, methods: data analysis, techniques: spectroscopic, turbulence, Astrophysics - Galaxy Astrophysics},
         year = 2010,
        month = feb,
       volume = {710},
       number = {1},
        pages = {853-858},
          doi = {10.1088/0004-637X/710/1/853},
archivePrefix = {arXiv},
       eprint = {arXiv:0905.4413},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...710..853C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2006ApJ...645L..25L,
       author = {{Lazarian}, A.},
        title = "{Enhancement and Suppression of Heat Transfer by MHD Turbulence}",
      journal = {ApJl},
     keywords = {Galaxies: Clusters: General, ISM: General, Magnetohydrodynamics: MHD, Turbulence, Astrophysics},
         year = 2006,
        month = jul,
       volume = {645},
       number = {1},
        pages = {L25-L28},
          doi = {10.1086/505796},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608045},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...645L..25L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021ApJ...911...37H,
       author = {{Hu}, Yue and {Xu}, Siyao and {Lazarian}, A.},
        title = "{Anisotropies in Compressible MHD Turbulence: Probing Magnetic Fields and Measuring Magnetization}",
      journal = {ApJ},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {911},
       number = {1},
          eid = {37},
        pages = {37},
          doi = {10.3847/1538-4357/abea18},
archivePrefix = {arXiv},
       eprint = {arXiv:2012.06039},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911...37H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019MNRAS.483.1287G,
       author = {{Gonz{\'a}lez-Casanova}, Diego F. and {Lazarian}, A. and {Burkhart}, Blakesley},
        title = "{Velocity centroid gradients for absorbing media}",
      journal = {MNRAS},
     keywords = {MHD, molecular data, turbulence, ISM: kinematics and dynamics, ISM: magnetic fields, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = feb,
       volume = {483},
       number = {1},
        pages = {1287-1294},
          doi = {10.1093/mnras/sty2775},
archivePrefix = {arXiv},
       eprint = {arXiv:1703.03035},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.483.1287G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019ApJ...873...16H,
       author = {{Hsieh}, Cheng-han and {Hu}, Yue and {Lai}, Shih-Ping and {Yuen}, Ka Ho and {Liu}, Sheng-Yuan and {Hsieh}, I. -Ta and {Ho}, Ka Wai and {Lazarian}, A.},
        title = "{Tracing Magnetic Field Morphology Using the Velocity Gradient Technique in the Presence of CO Self-absorption}",
      journal = {ApJ},
     keywords = {ISM: magnetic fields, ISM: molecules, magnetohydrodynamics: MHD, methods: numerical, radiative transfer, turbulence, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = mar,
       volume = {873},
       number = {1},
          eid = {16},
        pages = {16},
          doi = {10.3847/1538-4357/ab0376},
archivePrefix = {arXiv},
       eprint = {arXiv:1809.09806},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...873...16H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021MNRAS.502.1768H,
       author = {{Hu}, Yue and {Lazarian}, A.},
        title = "{A synergy of the velocity gradients technique and the probability density functions for identifying gravitational collapse in self-absorbing media}",
      journal = {MNRAS},
     keywords = {MHD, radiative transfer, turbulence, ISM: general, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {502},
       number = {2},
        pages = {1768-1784},
          doi = {10.1093/mnras/stab087},
archivePrefix = {arXiv},
       eprint = {arXiv:2001.05648},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.502.1768H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2020ApJ...897..123H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Yuen}, Ka Ho},
        title = "{Velocity Gradient in the Presence of Self-gravity: Identifying Gravity-induced Inflow and Determining Collapsing Stage}",
      journal = {ApJ},
     keywords = {845, 1569, 847, 1565, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = jul,
       volume = {897},
       number = {2},
          eid = {123},
        pages = {123},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2020RNAAS...4..105H,
       author = {{Hu}, Yue and {Lazarian}, A.},
        title = "{Modeling of Galactic Foreground Polarization with Velocity Gradients}",
      journal = {Research Notes of the American Astronomical Society},
     keywords = {Interstellar medium, Interstellar magnetic fields, Interstellar dynamics, 847, 845, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jul,
       volume = {4},
       number = {7},
          eid = {105},
        pages = {105},
          doi = {10.3847/2515-5172/aba359},
archivePrefix = {arXiv},
       eprint = {arXiv:2007.02184},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020RNAAS...4..105H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021ApJ...911...53H,
       author = {{Ho}, Ka Wai and {Lazarian}, A.},
        title = "{Intermittency of Fast MHD Modes and Regions of Anomalous Gradient Orientation in Low-{\ensuremath{\beta}} Plasmas}",
      journal = {ApJ},
     keywords = {Interstellar magnetic fields, Interstellar medium, Interstellar dynamics, 845, 847, 839, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = apr,
       volume = {911},
       number = {1},
          eid = {53},
        pages = {53},
          doi = {10.3847/1538-4357/abe713},
archivePrefix = {arXiv},
       eprint = {arXiv:2104.08627},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...911...53H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022MNRAS.tmp.1055H,
       author = {{Hu}, Yue and {Lazarian}, A. and {Wang}, Q. Daniel},
        title = "{Decomposing magnetic fields in three dimensions over the central molecular zone}",
      journal = {MNRAS},
     keywords = {magnetic fields, turbulence, ISM: general, ISM: magnetic fields, Galaxy: centre, Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jul,
       volume = {513},
       number = {3},
        pages = {3493-3509},
          doi = {10.1093/mnras/stac1060},
archivePrefix = {arXiv},
       eprint = {arXiv:2201.07970},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022MNRAS.513.3493H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019ApJ...874..171C,
       author = {{Clark}, S.~E. and {Peek}, J.~E.~G. and {Miville-Desch{\^e}nes}, M. -A.},
        title = "{The Physical Nature of Neutral Hydrogen Intensity Structure}",
      journal = {ApJ},
     keywords = {dust, extinction, ISM: magnetic fields, ISM: structure, magnetic fields, radio lines: ISM, turbulence, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {874},
       number = {2},
          eid = {171},
        pages = {171},
          doi = {10.3847/1538-4357/ab0b3b},
archivePrefix = {arXiv},
       eprint = {arXiv:1902.01409},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...874..171C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019arXiv190403173Y,
       author = {{Yuen}, Ka Ho and {Hu}, Yue and {Lazarian}, A. and {Pogosyan}, D.},
        title = "{Comment on Clark et al. (2019) ``The Physical Nature of Neutral Hydrogen Intensity Structure''}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
          eid = {arXiv:1904.03173},
        pages = {arXiv:1904.03173},
archivePrefix = {arXiv},
       eprint = {arXiv:1904.03173},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190403173Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2021ApJ...910..161Y,
       author = {{Yuen}, Ka Ho and {Ho}, Ka Wai and {Lazarian}, Alex},
        title = "{Technique for Separating Velocity and Density Contributions in Spectroscopic Data and Its Application to Studying Turbulence and Magnetic Fields}",
      journal = {ApJ},
     keywords = {Interstellar magnetic fields, Interstellar medium, Interstellar dynamics, Interstellar atomic gas, Interstellar filaments, 845, 847, 839, 833, 842, Astrophysics - Astrophysics of Galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics, Physics - Data Analysis, Statistics and Probability, Physics - Fluid Dynamics},
         year = 2021,
        month = apr,
       volume = {910},
       number = {2},
          eid = {161},
        pages = {161},
          doi = {10.3847/1538-4357/abe4d4},
archivePrefix = {arXiv},
       eprint = {arXiv:2012.15776},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...910..161Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2022arXiv220512084T,
       author = {{Tram}, Le Ngoc and {Bonne}, Lars and {Hu}, Yue and {Lopez-Rodriguez}, Enrique and {Guerra}, Jordan A. and {Lesaffre}, Pierre and {Gusdorf}, Antoine and {Hoang}, Thiem and {Lee}, Min-Young and {Lazarian}, Alex and {Andersson}, B-G and {Coude}, Simon and {Soam}, Archana and {Vacca}, William D. and {Lee}, Hyeseung and {Gordon}, Michael},
        title = "{SOFIA observations of 30 Doradus: II -- Magnetic fields and large scale gas kinematics}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = may,
          eid = {arXiv:2205.12084},
        pages = {arXiv:2205.12084},
archivePrefix = {arXiv},
       eprint = {arXiv:2205.12084},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220512084T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022arXiv220606717Z,
       author = {{Zhao}, Mengke and {Zhou}, Jianjun and {Hu}, Yue and {Lazarian}, A. and {Tang}, Xindi and {Baan}, Willem A. and {Esimbek}, Jarken and {He}, Yuxin and {Li}, Dalei and {Ji}, Weiguang and {Tursun}, Kadirya},
        title = "{Magnetic Field of Molecular Gas Measured with the Velocity Gradient Technique I. Orion A}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = jun,
          eid = {arXiv:2206.06717},
        pages = {arXiv:2206.06717},
archivePrefix = {arXiv},
       eprint = {arXiv:2206.06717},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220606717Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2013ApJ...762L..27H,
       author = {{Hu}, Tao and {Shao}, Zhengyi and {Peng}, Qiuhe},
        title = "{New Estimates of the Inclination, Position Angle, Pitch Angle, and Scale Height of the Whirlpool Galaxy}",
      journal = {ApJL},
     keywords = {galaxies: individual: M51, galaxies: spiral, galaxies: structure},
         year = 2013,
        month = jan,
       volume = {762},
       number = {2},
          eid = {L27},
        pages = {L27},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...762L..27H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019ApJS..244...24L,
       author = {{Leroy}, Adam K. and {Sandstrom}, Karin M. and {Lang}, Dustin and {Lewis}, Alexia and {Salim}, Samir and {Behrens}, Erica A. and {Chastenet}, J{\'e}r{\'e}my and {Chiang}, I-Da and {Gallagher}, Molly J. and {Kessler}, Sarah and {Utomo}, Dyas},
        title = "{A z = 0 Multiwavelength Galaxy Synthesis. I. A WISE and GALEX Atlas of Local Galaxies}",
      journal = {ApJS},
     keywords = {galaxies: general, galaxies: ISM, galaxies: spiral, galaxies: star formation, infrared: galaxies, ultraviolet: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {244},
       number = {2},
          eid = {24},
        pages = {24},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJS..244...24L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019A&A...624A..80N,
       author = {{Nersesian}, A. and {Xilouris}, E.~M. and {Bianchi}, S. and {Galliano}, F. and {Jones}, A.~P. and {Baes}, M. and {Casasola}, V. and {Cassar{\`a}}, L.~P. and {Clark}, C.~J.~R. and {Davies}, J.~I. and {Decleir}, M. and {Dobbels}, W. and {De Looze}, I. and {De Vis}, P. and {Fritz}, J. and {Galametz}, M. and {Madden}, S.~C. and {Mosenkov}, A.~V. and {Tr{\v{c}}ka}, A. and {Verstocken}, S. and {Viaene}, S. and {Lianou}, S.},
        title = "{Old and young stellar populations in DustPedia galaxies and their role in dust heating}",
      journal = {AA},
     keywords = {dust, extinction, infrared: galaxies, galaxies: photometry, galaxies: ISM, galaxies: evolution, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = apr,
       volume = {624},
          eid = {A80},
        pages = {A80},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...624A..80N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017A&A...597A..85B,
       author = {{Beuther}, H. and {Meidt}, S. and {Schinnerer}, E. and {Paladino}, R. and {Leroy}, A.},
        title = "{Interactions of the Galactic bar and spiral arm in NGC 3627}",
      journal = {AA},
     keywords = {stars: formation, galaxies: individual: NGC 3627, stars: massive, ISM: clouds, ISM: structure, Astrophysics - Astrophysics of Galaxies},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A85},
        pages = {A85},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A..85B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2003A&A...407..485G,
       author = {{Garc{\'\i}a-Burillo}, S. and {Combes}, F. and {Hunt}, L.~K. and {Boone}, F. and {Baker}, A.~J. and {Tacconi}, L.~J. and {Eckart}, A. and {Neri}, R. and {Leon}, S. and {Schinnerer}, E. and {Englmaier}, P.},
        title = "{Molecular Gas in NUclei of GAlaxies (NUGA). I. The counter-rotating LINER NGC 4826}",
      journal = {AA},
     keywords = {galaxies: individual: NGC 4826, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, radio lines: galaxies, Astrophysics},
         year = 2003,
        month = aug,
       volume = {407},
        pages = {485-502},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...407..485G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2013ApJ...779...45M,
       author = {{Meidt}, Sharon E. and {Schinnerer}, Eva and {Garc{\'\i}a-Burillo}, Santiago and {Hughes}, Annie and {Colombo}, Dario and {Pety}, J{\'e}r{\^o}me and {Dobbs}, Clare L. and {Schuster}, Karl F. and {Kramer}, Carsten and {Leroy}, Adam K. and {Dumas}, Galle and {Thompson}, Todd A.},
        title = "{Gas Kinematics on Giant Molecular Cloud Scales in M51 with PAWS: Cloud Stabilization through Dynamical Pressure}",
      journal = {ApJ},
     keywords = {galaxies: individual: M51, galaxies: ISM, galaxies: star formation, ISM: kinematics and dynamics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2013,
        month = dec,
       volume = {779},
       number = {1},
          eid = {45},
        pages = {45},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2016A&A...588A..33Q,
       author = {{Querejeta}, M. and {Meidt}, S.~E. and {Schinnerer}, E. and {Garc{\'\i}a-Burillo}, S. and {Dobbs}, C.~L. and {Colombo}, D. and {Dumas}, G. and {Hughes}, A. and {Kramer}, C. and {Leroy}, A.~K. and {Pety}, J. and {Schuster}, K.~F. and {Thompson}, T.~A.},
        title = "{Gravitational torques imply molecular gas inflow towards the nucleus of M 51}",
      journal = {AA},
     keywords = {galaxies: individual: M 51, galaxies: ISM, galaxies: structure, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, Astrophysics - Astrophysics of Galaxies},
         year = 2016,
        month = apr,
       volume = {588},
          eid = {A33},
        pages = {A33},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1995AJ....110..156Q,
       author = {{Quillen}, A.~C. and {Frogel}, Jay A. and {Kuchinski}, L.~E. and {Terndrup}, D.~M.},
        title = "{Multiband Images of the Barred Galaxy NGC 1097}",
      journal = {AJ},
     keywords = {GALAXIES: INDIVIDUAL: NGC 1079, GALAXIES: ISM, GALAXIES: STELLAR CONTENT, Astrophysics},
         year = 1995,
        month = jul,
       volume = {110},
        pages = {156},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2009ApJ...702..114D,
       author = {{Davies}, R.~I. and {Maciejewski}, W. and {Hicks}, E.~K.~S. and {Tacconi}, L.~J. and {Genzel}, R. and {Engel}, H.},
        title = "{Stellar and Molecular Gas Kinematics Of NGC 1097: Inflow Driven by a Nuclear Spiral}",
      journal = {ApJ},
     keywords = {galaxies: active, galaxies: individual: NGC 1097, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: spiral, infrared: galaxies, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = sep,
       volume = {702},
       number = {1},
        pages = {114-128},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2010ApJ...723..767V,
       author = {{van de Ven}, Glenn and {Fathi}, Kambiz},
        title = "{Kinematic Analysis of Nuclear Spirals: Feeding the Black Hole in NGC 1097}",
      journal = {ApJ},
     keywords = {galaxies: active, galaxies: individual: NGC 1097, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: structure, Astrophysics - Galaxy Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics},
         year = 2010,
        month = nov,
       volume = {723},
       number = {1},
        pages = {767-780},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2014A&A...567A.125G,
       author = {{Garc{\'\i}a-Burillo}, S. and {Combes}, F. and {Usero}, A. and {Aalto}, S. and {Krips}, M. and {Viti}, S. and {Alonso-Herrero}, A. and {Hunt}, L.~K. and {Schinnerer}, E. and {Baker}, A.~J. and {Boone}, F. and {Casasola}, V. and {Colina}, L. and {Costagliola}, F. and {Eckart}, A. and {Fuente}, A. and {Henkel}, C. and {Labiano}, A. and {Mart{\'\i}n}, S. and {M{\'a}rquez}, I. and {Muller}, S. and {Planesas}, P. and {Ramos Almeida}, C. and {Spaans}, M. and {Tacconi}, L.~J. and {van der Werf}, P.~P.},
        title = "{Molecular line emission in NGC 1068 imaged with ALMA. I. An AGN-driven outflow in the dense molecular gas}",
      journal = {AA},
     keywords = {galaxies: individual: NGC 1068, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: nuclei, galaxies: Seyfert, radio lines: galaxies, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = jul,
       volume = {567},
          eid = {A125},
        pages = {A125},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...692.1623H,
       author = {{Haan}, Sebastian and {Schinnerer}, Eva and {Emsellem}, Eric and {Garc{\'\i}a-Burillo}, Santiago and {Combes}, Francoise and {Mundell}, Carole G. and {Rix}, Hans-Walter},
        title = "{Dynamical Evolution of AGN Host Galaxies{\textemdash}Gas In/Out-Flow Rates in Seven NUGA Galaxies}",
      journal = {ApJ},
     keywords = {accretion, accretion disks, galaxies: active, galaxies: individual: NGC3368 NGC3627 NGC4321 NGC4736 NGC5248 NGC6951 NGC7217, galaxies: ISM, galaxies: kinematics and dynamics, galaxies: Seyfert, radio lines: galaxies, Astrophysics},
         year = 2009,
        month = feb,
       volume = {692},
       number = {2},
        pages = {1623-1661},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2022arXiv220806090L,
       author = {{Liu}, Mingrui and {Hu}, Yue and {Lazarian}, A. and {Xu}, Siyao and {Soida}, Marian},
        title = "{Multi-Phase Magnetic Fields in the Galaxy NGC 3627}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies},
         year = 2022,
        month = aug,
          eid = {arXiv:2208.06090},
        pages = {arXiv:2208.06090},
archivePrefix = {arXiv},
       eprint = {2208.06090},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv220806090L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2021ApJ...908...12L,
       author = {{Lazarian}, A. and {Hoang}, Thiem},
        title = "{Alignment and Rotational Disruption of Dust}",
      journal = {\apj},
     keywords = {Interstellar medium, Astrosphere interstellar medium interactions, Interstellar dust, Interstellar dust extinction, Interstellar dust processes, Starlight polarization, Astrochemistry, 847, 106, 836, 837, 838, 1571, 75, Astrophysics - Astrophysics of Galaxies, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = feb,
       volume = {908},
       number = {1},
          eid = {12},
        pages = {12},
          doi = {10.3847/1538-4357/abd02c},
archivePrefix = {arXiv},
       eprint = {2010.15301},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJ...908...12L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

